Optimum Methods for Quasi-Orthographic Surface Imaging

The need for fast, effective and accurate surveys have become increasingly necessary. A major part of the research is supported by photographic surveys which are used for capturing expansive natural surfaces using a wide range of sensors -- visual, infrared, ultrasonic, radio, etc. Because of the unpredictability and fast-varying characteristic of natural surfaces, it is often very difficult to capture and reconstruct them accurately. Moreover, the non-smooth nature results in the occlusion of major areas when a small number of captures are used for reconstruction, resulting in loss of important and maybe significant information or surface features. In a perfect orthographic reconstruction, images must be captured normal to each point on the surface which is practically implausible. This thesis aims at proposing several algorithms for deciding optimal capture points, given a surface, such that the optimal captures can be used for an approximate orthographic reconstruction. An approximate orthographic capture has been attributed to a small field of view and a closed form relationship has been derived for evaluating local orthographic capture region which varies depending on the point of capture on the surface. Based on the formula to calculate approximate local orthographic regions, several algorithms have been developed using non-convex optimization techniques for covering the entire surface with minimum number of such capture points. The algorithms have been compared on the basis of accuracy and computational complexity and parameters have been tuned depending on the nature of the surface. A separate algorithm has been proposed to identify such capture points empirically depending on the local surface-curvatures. Given these algorithms, users can make informed choices regarding which to adopt in their application as per their requirements.

==> IIT_Kanpur_Thesis_Template/applications.tex <==
\chapter{Experiences and applications}

In this chapter we discuss the lessons we
have learnt and a few ideas we have explored.

\section{Title}
\label{sec:quantified}


\subsection*{Summary}

Write your summary here.


==> IIT_Kanpur_Thesis_Template/conclusions.tex <==
\chapter{Conclusions}

Our implementation is open source and freely available at
\begin{center}
\url{http://www.cse.iitk.ac.in/users/karkare/code/z3.rkt/}
\end{center}

\section{Scope for further work}

In the long term, we hope the community will find this system useful and will
contribute to the project to solve large practical problems.


==> IIT_Kanpur_Thesis_Template/intro.tex <==
\chapter{Introduction}
\label{chap:intro}

\section{Section 1}

\section{Section 2}


==> IIT_Kanpur_Thesis_Template/prelude.tex <==
% prelude.tex
%   - titlepage
%   - dedication (optional)
%   - approval sheet
%   - course certificate
%   - table of contents, list of tables and list of figures
%   - nomenclature
%   - abstract
%============================================================================


\clearpage\pagenumbering{roman}  % This makes the page numbers Roman (i, ii, etc)



% TITLE PAGE
%   - define \title{} \author{} \date{}
\title{Thesis Title}
\author{Author Name}
\date{June, 2012}

%  - Roll number, required for title page, approval sheet, and
%    certificate of course work 
\rollnum{Y799999} 

%   - The default degree is ``Doctor of Philosophy''
%     (unless the document style msthesis is specified
%      and then the default degree is ``Master of Science'')
%     Degree can be changed using the command \iitbdegree{}
\iitbdegree{Master of Technology}

%   - The default report type is preliminary report.
%      * for a PhD thesis, specify \thesis
\thesis
%      * for a M.Tech./M.Phil./M.Des./M.S. dissertation, specify \dissertation
%\dissertation
%      * for a DIIT/B.Tech./M.Sc.project report, specify \project
%\project
%      * for any other type, use  \reporttype{}
%\reporttype{ReportType}

%   - The default department is ``Unknown Department''
%     The department can be changed using the command \department{}
\department{Computer Science \& Engineering}

%    - Set the guide's name
\setguide{Prof Amey Karkare}
\setguidedept{Department of Computer Science \& Engineering}

%   - once the above are defined, use \maketitle to generate the titlepage
\maketitle

%--------------------------------------------------------------------%
% CERTIFICATE
%     The first page after the title page.
\makecertificate

%--------------------------------------------------------------------%
% COPYRIGHT PAGE
%   - To include a copyright page use \copyrightpage
% \copyrightpage

%--------------------------------------------------------------------%
% ABSTRACT
\begin{abstract}
Abstract not more that 300 words
\end{abstract}

%--------------------------------------------------------------------%
% DEDICATION
%   Dedications, if any.
\begin{dedication}
To my grandfather
\end{dedication}

% Acknowledgements
\begin{acknowledgments}

I would like to thank all the people who helped me during my thesis.

\end{acknowledgments}

%--------------------------------------------------------------------%
% CONTENTS, TABLES, FIGURES
\tableofcontents
\listoftables

\cleardoublepage
\phantomsection \label{listoffig}
\addcontentsline{toc}{chapter}{List of Figures}
\listof{program}{List of Figures}
%\listoffigures

\cleardoublepage\pagenumbering{arabic} % Make the page numbers Arabic (1, 2, etc)


==> IIT_Kanpur_Thesis_Template/prelude_synopsis.tex <==
% prelude.tex
%   - titlepage
%   - dedication (optional)
%   - approval sheet
%   - course certificate
%   - table of contents, list of tables and list of figures
%   - nomenclature
%   - abstract
%============================================================================


\clearpage\pagenumbering{roman}  % This makes the page numbers Roman (i, ii, etc)



% TITLE PAGE
%   - define \title{} \author{} \date{}
\title{How to \LaTeX\ a Thesis}
\author{Amey Karkare}
\date{2007}

%  - Roll number, required for title page, approval sheet, and
%    certificate of course work 
\rollnum{02405003} 

%   - The default degree is ``Doctor of Philosophy''
%     (unless the document style msthesis is specified
%      and then the default degree is ``Master of Science'')
%     Degree can be changed using the command \degree{}
\iitbdegree{Doctor of Philosophy}

%   - The default report type is preliminary report.
%      * for a PhD thesis, specify \thesis
%\thesis
%      * for a M.Tech./M.Phil./M.Des./M.S. dissertation, specify \dissertation
%\dissertation
%      * for a DIIT/B.Tech./M.Sc.project report, specify \project
%\project
%      * for any other type, use  \reporttype{}
\reporttype{synopsis}

%   - The default department is ``Unknown Department''
%     The department can be changed using the command \department{}
\department{DEPARTMENT OF COMPUTER SCIENCE \& ENGINEERING}

%    - Set the guide's name
\setguide{Prof My Guide}
%    - Set the coguide's name (if you have one)
%\setcoguide{Prof Co Guide}
%    - Set external guide (if you have one)
%\setexguide{Prof External Guide}

%   - once the above are defined, use \maketitle to generate the titlepage
\maketitle



==> IIT_Kanpur_Thesis_Template/related.tex <==
\chapter{Related work}

Related work goes here


==> IIT_Kanpur_Thesis_Template/technical.tex <==
\chapter{Design and implementation}
\label{chap:design-impl}

Implementation details go here.

